Data-Driven Crowd Simulation with Generative Adversarial Networks

This paper presents a novel data-driven crowd simulation method that can mimic the observed traffic of pedestrians in a given environment. Given a set of observed trajectories, we use a recent form of neural networks, Generative Adversarial Networks (GANs), to learn the properties of this set and generate new trajectories with similar properties. We define a way for simulated pedestrians (agents) to follow such a trajectory while handling local collision avoidance. As such, the system can generate a crowd that behaves similarly to observations, while still enabling real-time interactions between agents. Via experiments with real-world data, we show that our simulated trajectories preserve the statistical properties of their input. Our method simulates crowds in real time that resemble existing crowds, while also allowing insertion of extra agents, combination with other simulation methods, and user interaction.

==> emd.tex <==
\subsection{Descriptors} 
There are multiple ways to describe the properties of a crowd and therefore to compare two crowds (real or simulated). Here is a short-list of well-known descriptors:


\begin{enumerate}
	\item Heatmap: By collecting all the locations of the agents during whole the experiment, we can find the spatial distribution of agents. Parzen Window can be used to estimate the distribution. 
	
	\item Fundamental Diagram: This descriptor is inspired by the field of pedestrian dynamics where it computes the speed of an agent in a given local density, form up a set of pairs of (v, d) and then provides a distribution of this 2d samples. 
	
	\item Vorticity: It describes the local spinning motion of a crowd near a point.
	
	\item Distribution of Inter-Pedestrian Distances: Computing the distance between every pair of agents, we can estimate the IPD distribution. \\	
	\CommentJavad{I think PCF (pair correlation function or Radial Distribution Function) which Pierre was using also makes sense.}
	
\end{enumerate}

In this work we propose to use Earth Mover's Distance to measure the similarity between two given experiments. \\
\CommentJavad{I feel it is not used in Crowd Simulation Community and can be of our contributions} \\
\CommentJavad{Explain why above descriptors can not capture all relevant information from crowd (maybe with simple counterexamples)}

\subsection{Earth Mover's Distance}

Generally the Earth Mover's Distance (EMD) is a method to evaluate dissimilarity between two multi-dimensional distributions in some feature space where a \textit{ground distance} is defined to measure the distance between a pair of features. 

\CommentJavad{I'd like to have a better similarity function between trajectories. DTW is a suitable and well-known metric, but there are two problems: Does not satisfy triangular inequality and identity of indiscernibles. By adding the length difference of the trajectories the 2nd condition will be satisfied.}

\begin{equation}
	d({\mathbf{x}}^i_{1:T_i}, {\mathbf{x}}^j_{1:T_j}) = DTW({\mathbf{x}}^i_{1:T_i}, {\mathbf{x}}^j_{1:T_j}) 
	+ \lambda | T_i - T_j |
\label{dtw_eq}
\end{equation}

We added this second term in equation \ref{dtw_eq} to solve the problem of identity of indiscernibles of DTW similarity measure ...


%To compute the distance between two given trajectories ${{\mathbf{x}}^i_{1:T_i}}$ and ${{\mathbf{x}}^j_{1:T_j}}$ with lengths of $T_i$ and $T_i$, respectively, we consider two aspects of the samples:  spatial difference and average speed difference. Consider among these two samples the longer sample ${\mathbf{x}}^L$ and the shorter one ${\mathbf{x}}^S$ :

%\begin{equation}
%\begin{split}
%&T^L = \max (T_i~,~T_j)\\
%&{\mathbf{x}}^L = \argmax_{\mathbf{x}^i, \mathbf{x}^j} (T_i~,~T_j)\\
%&{\mathbf{x}}^S = \argmin_{\mathbf{x}^i, \mathbf{x}^j} (T_i~,~T_j)
%\end{split}
%\end{equation}


%Then we augment ${\mathbf{x}}^S$ with interpolated points \textcolor{red}{to be explained} to convert it to a trajectory with the same size as the longer sample $T^L$. The augmented trajectory is denoted as $\mathbf{x'}^S$.

%Then the spatial difference is defined as follows:
%\begin{equation}
%d_p = \sum_{t=1}^{T_L} \lVert \mathbf{x}^L_t - \mathbf{x}'^S_t \rVert
%\label{eq:spatial_diff}
%\end{equation}

%The speed difference is calculated as below:
%\begin{equation}
%	d_s = \lVert \dfrac{\sum_{t=1}^{T_i-1} \lVert {\mathbf{x}^i_{t+1} - \mathbf{x}^i_{t}} \rVert} {T_i - 1} 
%	- \dfrac{\sum_{t=1}^{T_j-1} \lVert {\mathbf{x}^j_{t+1} - \mathbf{x}^j_{t}} \rVert} {T_j - 1} \rVert
%\end{equation}

%The ground distance will be then:
%\begin{equation}
%	d = d_p + \lambda d_s
%\end{equation}


The Wasserstein distance between two distribution of trajectories $\mathbf{X}$, $\mathbf{Y}$ will be:

\begin{equation}
	d(\mathbf{X}, \mathbf{Y}) = 
	\inf_{\gamma \in \Gamma(\mathbf{X}, \mathbf{Y})} ~\mathbb{E}_{(\mathbf{x}, ~\mathbf{y}) \sim \gamma}
	[{d(\mathbf{x}, \mathbf{y})}]
\label{emd_eq}
\end{equation}

where $\Gamma(\mathbf{X}, \mathbf{Y})$ denotes the set of all joint distributions of $\mathbf{X}$ and $\mathbf{Y}$ and $\mathbf{x}$ and $\mathbf{y}$ are samples from $\mathbf{X}, \mathbf{Y}$, respectively. 

As we dont have the distributions directly, and instead we work with two given sets of samples $X$ and $Y$ containing $m$ and $n$ samples, respectively, hence the actual EMD can be computed as follows:

\begin{equation}
\begin{split}
	&EMD(X, Y) = \min_{w \in \mathbb{R}^{n \times m}}
	\sum_{i=1}^{n} \sum_{j=1}^{m}
	w^{ij} d(\mathbf{x}^i, ~\mathbf{y}^j)		\\
	s.t.\\
	& w^{ij} >= 0, ~1 \leq i \leq n, ~ 1 \leq j \leq m \\
	& \sum_{j=1}^m w^{ij} = 1/n, ~1 \leq i \leq n\\
	& \sum_{i=1}^n w^{ij} = 1/m, ~1 \leq j \leq m
\end{split}
\end{equation}

For sake of simplicity, we assume $n=m$ i.e. the number of samples in two given sets should be equal.

\CommentJavad{I need to find out its connection with Hungarian algorithm, which solves the assignment problem http://smat.epfl.ch/~zemel/vt/pdm.pdf}\\
\CommentJavad{Wiki: Hungarian algorithm can be used to get the solution if the domain D is the set {0,1}. If the domain is integral, it can be translated for the same algorithm by representing integral bins as multiple binary bins.}
